WeCromCL: Weakly Supervised Cross-Modality Contrastive Learning for Transcription-only Supervised Text Spotting

Transcription-only Supervised Text Spotting aims to learn text spotters relying only on transcriptions but no text boundaries for supervision, thus eliminating expensive boundary annotation. The crux of this task lies in locating each transcription in scene text images without location annotations. In this work, we formulate this challenging problem as a Weakly Supervised Cross-modality Contrastive Learning problem, and design a simple yet effective model dubbed WeCromCL that is able to detect each transcription in a scene image in a weakly supervised manner. Unlike typical methods for cross-modality contrastive learning that focus on modeling the holistic semantic correlation between an entire image and a text description, our WeCromCL conducts atomistic contrastive learning to model the character-wise appearance consistency between a text transcription and its correlated region in a scene image to detect an anchor point for the transcription in a weakly supervised manner. The detected anchor points by WeCromCL are further used as pseudo location labels to guide the learning of text spotting. Extensive experiments on four challenging benchmarks demonstrate the superior performance of our model over other methods. Code will be released.

==> tables/full_supervised_methods.tex <==
\begin{table}%\scalebox{0.7}
  \caption{\wu{Effectiveness of proposed \emph{\mymodel}  on fully supervised text spotting method.}}
   \label{tab:fully_supervised}
  \begin{tabular}{l|ccc|cc}
   \toprule
   \multirow{2}{*}{Training Data} &   \multicolumn{2}{c}{End-to-end}\\
   & None & Full\\
   
  \hline
   GT & 78.2 & 86.7\\
   GT + ArT pseudo labels (50\%) &78.6
 & \textbf{86.8}\\
   GT + ArT pseudo labels (100\%)& \textbf{78.7}
& \textbf{86.8}\\
  \bottomrule
\end{tabular}
\end{table}

==> tables/pseudo_label.tex <==
\begin{table*}%\scalebox{0.7}
  \caption{Quantitative evaluation results of the generated pseudo labels.} 
   \label{tab:pseudo}
  \begin{tabular}{l|ccc|ccc|ccc|ccc}
   \toprule
   \multirow{2}{*}{Inference set} & \multicolumn{3}{c|}{ICDAR 2013} &  \multicolumn{3}{c|}{ICDAR 2015}&  \multicolumn{3}{c|}{Total-Text} &  \multicolumn{3}{c}{CTW1500}\\
   \cmidrule(lr){2-13}
   & P & R & F& P & R & F& P & R & F& P & R & F\\
   
  \hline
   Training set &93.2 &93.2 &93.2 & 91.4 & 86.0 & 88.6& 83.5 & 85.1 & 84.3 & 67.0 & 65.7 & 66.3\\
   Testing set  &90.4 &90.5 &90.5 & 86.9 & 80.1 & 83.4 & 85.8 & 75.4 & 80.3 & 78.9 & 76.5 & 77.7\\
  \bottomrule
\end{tabular}
\end{table*}

==> tables/retrieval.tex <==

\begin{table}
  \caption{Quantitative results on scene text retrieval task.} 
  %\vspace{-6pt}
  \label{tab:retrieval}
  \begin{tabular}{l|ccc}
   \toprule
   Method & SVT & STR & CTR\\
  \hline
  \multicolumn{4}{c}{Scene Text Retrieval Methods}\\
  \hline
  Mishra \textit{et al.}~\cite{mishra2013image} &56.24&42.70& - \\
  Gomez \textit{et al.}~\cite{gomez2018single} &83.74& 69.83& 41.05\\
  Mafla \textit{et al.}~\cite{mafla2021real} & 85.74 &71.67 &-\\
  Wang \textit{et al.}~\cite{wang2021scene} &\textbf{89.38}& \textbf{77.09}& \textbf{66.45}\\
  \hline
  \multicolumn{4}{c}{Scene Text Spotting Methods}\\
   \hline
   
  Jaderberg \textit{et al.}~\cite{jaderberg2016reading} &86.30 &66.50 &-\\
  He \textit{et al.}~\cite{he2018end} (dictionary) & 80.54& 66.95& -\\
  ABCNet~\cite{liu2020abcnet} & 82.43& 67.25&- \\
  Mask Textspotter v3~\cite{liao2020mask} &84.54&\textbf{74.48}& 55.54\\  
  Ours&\textbf{86.37}& 66.68	&\textbf{57.80}\\
  %86.366	66.68	57.8
  \hline
 \makecell[l]{\emph{\mymodel}}&76.65& 57.46& 37.12 \\
  \bottomrule
\end{tabular}
\end{table}

==> tables/spotting.tex <==

\begin{table*}

\begin{minipage}{\linewidth}
\begin{minipage}[t]{0.55\linewidth}%minipage大小
\makeatletter\def\@captype{table}
\centering
\caption{Quantitative results on ICDAR 2013, ICDAR 2015, Total-Text and CTW1500. `*' denotes the performance evaluated by single-point metric. `$\dagger$' means the performance evaluated by edit-distance metric.} 
  %\vspace{-10pt}
  \label{tab:spotting}

\resizebox{1\linewidth}{!}{%表格大小
  \begin{tabular}{l|ccc|ccc|cc|cc}
  
   \toprule
   \multirow{2}{*}{Methods} & \multicolumn{3}{c|}{ICDAR 2013} &  \multicolumn{3}{c|}{ICDAR 2015}&  \multicolumn{2}{c|}{Total-Text} &  \multicolumn{2}{c}{CTW1500}\\
   \cmidrule(lr){2-11}
   & S & W & G& S & W & G& None & Full & None & Full\\
  \midrule
  \multicolumn{11}{c}{Fully Supervised Methods}\\
  \midrule
  MTS v3~\cite{liao2020mask}&-&-&-& 83.3& 78.1& 74.2&71.2& 78.4&-&-\\
  MANGO~\cite{qiao2020mango} &93.4 &92.3 &88.7&85.4& 80.1& 73.9&72.9& 83.6&58.9 &78.7 \\

  ABCNet v2~\cite{liu2021abcnet}&-&-&-& 82.7& 78.5& 73.0&70.4& 78.1& 57.5& 77.2\\
  TESTR~\cite{zhang2022text}&-&-&-&85.2& 79.4& 73.6&73.3 & 83.9&56.0& 81.5\\
  %SRSTS v2~\cite{wu2023single}&-&-&-&{86.5}& {82.4}&{78.1}&{82.1}& {88.1}&61.2& 83.5\\
  TTS ~\cite{kittenplon2022towards} & - & - & - &85.2 &81.7& 77.4&78.2& 86.3& - & -\\
  ABINet++~\cite{fang2022abinet++} & - & - & -&  84.1 &80.4 &75.4 &  77.6 &84.5& 60.2& 80.3\\
  Deepsolo~\cite{ye2023deepsolo} & - & - & - &86.8 &81.9 &76.9 &  79.7 &87.0 &64.2 &81.4\\
  ESTextSpotter~\cite{huang2023estextspotter} &- & - & - &87.5 &83.0& 78.1& 80.8 &87.1& 64.9 &83.9\\
  SPTS$^{*}$~\cite{peng2022spts}&93.3 &91.7 &88.5 &77.5 & 70.2& 65.8&74.2 &82.4&{63.6}&{83.8}\\
  SPTS v2${*}$~\cite{liu2023spts} & 93.9& 91.8 &88.6& 82.3& 77.7& 72.6&75.5 &84.0& 63.6& 84.3 \\
  \midrule
  \multicolumn{11}{c}{Semi-supervised Methods}\\
  \hline
  TTS$_\text{weak}$ ~\cite{kittenplon2022towards}&- & - & - & 78.7 &75.2& 70.1 & 75.1 & 83.5 & - & -\\
  \hline
  \multicolumn{11}{c}{Transcription-only Supervised Methods}\\
  \midrule
  TOSS$^{*}$ ~\cite{tang2022you} & 86.4&85.1& 82.2 & 65.9&59.6&52.4&65.1&74.8&\textbf{54.2}&65.3\\
\textbf{\mymodel + SRSTS-A}$^{*}$ & \textbf{89.9}&\textbf{88.1}&\textbf{83.7}&\textbf{82.1}&\textbf{76.1}&\textbf{68.8}&\textbf{70.1}&\textbf{81.4}&51.2&\textbf{75.7}\\
 \midrule
  NPTS$\dagger$ ~\cite{peng2022spts} & 89.6 &86.4 & 83.2 & 70.3 &62.7 &57.0 & 61.6 & 70.6 &50.9 & 70.5
 \\
  \textbf{\mymodel + SRSTS-A} $\dagger$  &\textbf{91.2}& \textbf{89.8}& \textbf{84.6}& \textbf{79.5}& \textbf{72.8}& \textbf{66.2}& \textbf{68.1}& \textbf{79.1}& \textbf{52.7}& \textbf{79.9}\\

  \bottomrule
\end{tabular}
}

\end{minipage}\quad
\begin{minipage}[t]{0.43\linewidth}%minipage大小
\makeatletter\def\@captype{table}
\centering

\caption{Performance comparison with previous scene text retrieval methods and scene text spotters. The metric for evaluation is mean average precision on `SVT', `STR' and `CTR'.} 
  %\vspace{-8pt}
  \label{tab:retrieval}
  \resizebox{0.86\linewidth}{!}{%表格大小
  \begin{tabular}{l|ccc}
   \toprule
   Method & SVT & STR & CTR\\
  \hline
  \multicolumn{4}{c}{Scene Text Spotters}\\
   \hline
   
  Jaderberg \textit{et al.}~\cite{jaderberg2016reading} &86.30 &66.50 &-\\
  He \textit{et al.}~\cite{he2018end} (dictionary) & 80.54& 66.95& -\\
  ABCNet~\cite{liu2020abcnet} & 82.43& 67.25&- \\
  MTS v3~\cite{liao2020mask} &84.54& \textbf{74.48}& 55.54\\  
  \textbf{\mymodel + SRSTS-A}&\textbf{88.37}& 72.32 &\textbf{60.04}\\
  %81.524	68.65	51.26
  %87.43	74.4834	62.58
  \hline
 \makecell[l]{\emph{\mymodel} (the first stage)}&81.52& 68.65& 51.26 \\
  \bottomrule
\end{tabular}
}
\end{minipage}
\end{minipage}
%\vspace{-10pt}
\end{table*}















